Probing Neutrino Oscillations with Reactor Antineutrinos in JUNO

The Jiangmen Underground Neutrino Observatory (JUNO) is a multi-purpose neutrino experiment currently under construction in South China, in an underground laboratory with approximately 650 m of rock overburden (1800 m.w.e.). The detector consists of a 20 kton liquid scintillator target, contained inside a 35.4-meter-diameter spherical acrylic vessel. The central detector (CD) is equipped with 17,612 20-inch and 25,600 3-inch Photomultipliers Tubes (PMTs), providing more than 75% total photocathode coverage. JUNO's main goal is the determination of the neutrino mass ordering with reactor antineutrinos, emitted from two adjacent nuclear power plants on a ~52.5 km baseline from the experimental site. JUNO's strategic location at a baseline corresponding to the first solar oscillation maximum, where the kinematic phase $\Delta_{21} \simeq \frac{\pi}{2}$, grants it the unique capability to simultaneously probe the effects of oscillations on both solar and atmospheric scales; moreover, it stands out as the first experiment to address the unresolved NMO question through vacuum-dominant oscillations. The oscillated energy spectrum in JUNO changes subtly depending on the neutrino mass ordering, which manifests as an energy-dependent phase shift, thus providing sensitivity to this parameter. Furthermore, the unparalleled size and energy resolution will enable to achieve a sub-percent precision on three parameters: $\Delta m_{21}^{2}$, $\Delta m_{31}^{2}$, and $\sin^2\theta_{12}$. This contribution will focus on JUNO's oscillation physics potential with reactor antineutrinos, with a particular emphasis on its crucial role in inaugurating a new era of precision within the neutrino sector.

==> bib.tex <==
@article{bib:reines-cowan,
  title={Detection of the free neutrino: a confirmation},
  author={Cowan Jr, Clyde L and Reines, Frederick and Harrison, FB and Kruse, HW and McGuire, AD},
  journal={Science},
  volume={124},
  number={3212},
  pages={103--104},
  year={1956},
  publisher={American Association for the Advancement of Science}
}

@article{bib:junophysics,
  title={{JUNO} physics and detector},
  author={Abusleme, A. and others},
  journal={Progress in Particle and Nuclear Physics},
  pages={103927},
  volume = {123},
  year={2021},
  publisher={Elsevier}
}


@article{bib:calibration,
  title={Calibration strategy of the {JUNO} experiment},
  author={Abusleme, A. and others},
  journal={Journal of High Energy Physics},
  volume={2021},
  number={3},
  pages={1--33},
  year={2021},
  publisher={Springer}
}


@article{bib:sub_osc,
  title={Sub-percent precision measurement of neutrino oscillation parameters with {JUNO}},
  author={Abusleme, A. and others},
  journal={Chinese Physics C},
  volume={46},
  number={12},
  pages={123001},
  year={2022},
  publisher={IOP Publishing}
}

@article{bib:tao,
  title={{TAO} conceptual design report: a precision measurement of the reactor antineutrino spectrum with sub-percent energy resolution},
  author={Abusleme, A. and others},
  journal={arXiv:2005.08745},
  year={2020}
}

@article{bib:dayabayNLcurves,
  title={A high precision calibration of the nonlinear energy response at {Daya Bay}},
  author={Adey, D. and others},
  journal={Nuclear Instruments and Methods in Physics Research Section A},
  volume={940},
  pages={230--242},
  year={2019},
  publisher={Elsevier}
}

@online{bib:mo,
  author       = {Jie Zhao},
  title        = {{JUNO Status \& Prospects}},
  month        = jun,
  year         = 2022,
  publisher    = {Zenodo},
  doi          = {10.5281/zenodo.6683749},
  url          = {https://doi.org/10.5281/zenodo.6683749}
}


@book{bib:giunti,
  title={Fundamentals of neutrino physics and astrophysics},
  author={Giunti, Carlo and Kim, Chung W},
  year={2007},
  publisher={Oxford university press}
}

@article{bib:pmns,
  title={Remarks on the unified model of elementary particles},
  author={Maki, Ziro and Nakagawa, Masami and Sakata, Shoichi},
  journal={Progress of Theoretical Physics},
  volume={28},
  number={5},
  pages={870--880},
  year={1962},
  publisher={Oxford University Press}
}

@article{bib:pdg,
    author = "P.A. Zyla et al.",
    collaboration = "Particle Data Group",
    title = "{Review of Particle Physics}",
    journal = {Progress of Theoretical and Experimental Physics},
    volume = {2020},
    number = {8},
    pages = {083C01},
    year = {2020},
    month = {08},
}


P.A. Zyla et al. (Particle Data Group), Prog. Theor. Exp. Phys. 2020, 083C01 (2020)

@article{bib:matterJUNO,
  title={Terrestrial matter effects on reactor antineutrino oscillations at {JUNO} or {RENO}-50: how small is small?},
  author={Li, Yufeng and Wang, Yifang and Xing, Zhizhong},
  journal={Chinese Physics C},
  volume={40},
  number={9},
  pages={091001},
  year={2016},
  publisher={IOP Publishing}
}

@article{bib:msw,
  title={The {LMA MSW} solution of the solar neutrino problem, inverted neutrino mass hierarchy and reactor neutrino experiments},
  author={Petcov, ST and Piai, M},
  journal={Physics Letters B},
  volume={533},
  number={1-2},
  pages={94--106},
  year={2002},
  publisher={Elsevier}
}


@article{bib:graphics,
  title={Unified graphical summary of neutrino mixing parameters},
  author={Mena, Olga and Parke, Stephen},
  journal={Physical Review D},
  volume={69},
  number={11},
  pages={117301},
  year={2004},
  publisher={APS}
}
